Distributional neural networks for electricity price forecasting

We present a novel approach to probabilistic electricity price forecasting which utilizes distributional neural networks. The model structure is based on a deep neural network that contains a so-called probability layer. The network's output is a parametric distribution with 2 (normal) or 4 (Johnson's SU) parameters. In a forecasting study involving day-ahead electricity prices in the German market, our approach significantly outperforms state-of-the-art benchmarks, including LASSO-estimated regressions and deep neural networks combined with Quantile Regression Averaging. The obtained results not only emphasize the importance of higher moments when modeling volatile electricity prices, but also -- given that probabilistic forecasting is the essence of risk management -- provide important implications for managing portfolios in the power sector.

==> fig/layers_table.tex <==
\begin{table*}[t!]
\caption{Activation functions and number of neurons selected in each of the hyperparameter tunings.}
	\centering
	\resizebox{\textwidth}{!}{
\begin{tabular}{|cr|rrrr|rrrr|rrrr|}
  \hline
  & & \multicolumn{4}{c|}{NN-Point} &  \multicolumn{4}{c|}{probNN-N} &  \multicolumn{4}{c|}{probNN-JSU}\\
 & Run &    1 &    2 &    3 &    4 &   1 &   2 &   3 &   4 &      1 & 2 &      3 &      4 \\
  \hline
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Layer 1}}} & Activation &  softplus &  softplus &  softplus &  softplus &  softplus &  softplus &  softplus &  softplus &  softplus &  elu &  softplus &  softplus \\
& Neurons    &       906 &       912 &       979 &       965 &       948 &       266 &       542 &       110 &       565 &  940 &       243 &       123 \\
\hline
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Layer 2}}} & Activation &  softplus &  softplus &      relu &       elu &       elu &      relu &  softplus &      relu &      relu &  elu &       elu &       elu \\
& Neurons    &       901 &       619 &       767 &       448 &       554 &       883 &       641 &       823 &       962 &   58 &       895 &       668 \\
  \hline
\end{tabular}
}
\label{tab:hyperpar_layers}
\end{table*}

